Scalar and Vector Airborne Platform Calibration Using Quantum and Classical Magnetometers and Inertial Sensors

Airborne magnetometry requires rigorous calibration to isolate geomagnetic signals from sensor errors and platform magnetic fields. This magnetic compensation is needed for applications like geophysical exploration and magnetic anomaly navigation. The standard approach utilizes a quantum scalar Optically Pumped Magnetometer (OPM) and a less sensitive fluxgate vector sensor for attitude information. This configuration typically results in a scalar approximation of the platform field. Advancements in high-sensitivity Diamond Nitrogen-Vacancy (NV) vector magnetometers now enable a re-evaluation of the standard hardware configuration and full vector calibration models. We show through rigorous theoretical analysis that scalar calibration models are robust to misalignment. Vector calibration models, however, are intrinsically first-order sensitive to attitude errors, irrespective of the accuracy of the magnetic field measurements. These errors arise from inaccurate representation of the background field direction in the body frame, and can amplify small orientation errors into noticeable calibration residuals. Using realistic sensor models and flight trajectories, we evaluate different sensor configurations for magnetic calibration and assess the use of onboard Inertial Navigation Systems (INS) as an independent attitude reference to enable stable compensation. Our results suggest that quantum vector magnetometers like NV sensors are not sufficient to solve the attitude bottleneck for airborne vector magnetic calibration. However, as a single sensor capable of providing both absolute field and directional measurements, they may offer benefits regarding sensor placement, synchronization, and scalar calibration accuracy.

==> appendices.tex <==
\section{}
\label{app:induced}
The induced coefficient term $B^p_{ind}$ in the scalar \ac{TL}-approximation can be rewritten to:
\begin{equation}
\begin{split}
    B^p_{ind} &=  \bfN  \bfB_e^b \cdot \hbfB_e^b = \begin{pmatrix}
    \beta_1 & \beta_2 & \beta_3 \\ \beta_4 & \beta_5 & \beta_6 \\ \beta_7 & \beta_8 & \beta_9 \end{pmatrix}  \bfB_e^b \cdot \hbfB_e^b \\
    &= \dfrac{1}{\left \lVert\bfB_e\right \rVert}\begin{pmatrix}
    \beta_1 B_x + \beta_2 B_y + \beta_3 B_z \\ \beta_4 B_x + \beta_5 B_y + \beta_6 B_z\\ \beta_7 B_x + \beta_8 B_y + \beta_9 B_z \end{pmatrix} \cdot \begin{pmatrix}
    B_x  \\ B_y \\  B_z \end{pmatrix} \\
    % USE \bigg HERE INSTEAD OF \left
    &= \dfrac{1}{\left \lVert\bfB_e\right \rVert} \biggl( \beta_1 B_x^2 + \beta_2 B_y B_x + \beta_3 B_z B_x + \beta_4 B_xB_y \\
    &\quad + \beta_5 B_y^2 + \beta_6 B_z B_y + \beta_7 B_x B_z + \beta_8 B_y B_z + \beta_9 B_z^2 \biggr)  \\
    &= \dfrac{1}{\left \lVert\bfB_e\right \rVert} \biggl( \beta_1 B_x^2 + (\beta_2 + \beta_4) B_x B_y + (\beta_3 + \beta_7) B_x B_z \\
    &\quad + \beta_5 B_y^2 + (\beta_6+\beta_8) B_y B_z + \beta_9 B_z^2\biggr) \\
    &=\begin{pmatrix}
    \beta_1 & (\beta_2 + \beta_4) & (\beta_3 + \beta_7) \\ 0 & \beta_5 & (\beta_6 + \beta_8) \\  0 & 0 & \beta_9 \end{pmatrix}  \bfB_e^b \cdot \hbfB_e^b.
\end{split}
\label{eq:B_p_ind}
\end{equation}
%
By defining $b_1 = \beta_1 $, $b_2 = \beta_2 + \beta_4 $, $b_3 = \beta_3 + \beta_7 $, $b_4 = \beta_5$,  $b_5 = \beta_6 + \beta_8$, $b_6 = \beta_9$, we end at
\begin{equation}
    B^p_{ind} =  \begin{pmatrix}
    b_1 & b_2 & b_3 \\ 0 & b_4 & b_5 \\ 0 & 0 & b_6
    \end{pmatrix}  \bfB_e^b \cdot \hbfB_e^b.
\end{equation}


% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
%\section{}
%Appendix two text goes here.
